LLMs are Vulnerable to Malicious Prompts Disguised as Scientific Language

As large language models (LLMs) have been deployed in various real-world settings, concerns about the harm they may propagate have grown. Various jailbreaking techniques have been developed to expose the vulnerabilities of these models and improve their safety. This work reveals that many state-of-the-art LLMs are vulnerable to malicious requests hidden behind scientific language. Specifically, our experiments with GPT4o, GPT4o-mini, GPT-4, LLama3-405B-Instruct, Llama3-70B-Instruct, Cohere, Gemini models demonstrate that, the models' biases and toxicity substantially increase when prompted with requests that deliberately misinterpret social science and psychological studies as evidence supporting the benefits of stereotypical biases. Alarmingly, these models can also be manipulated to generate fabricated scientific arguments claiming that biases are beneficial, which can be used by ill-intended actors to systematically jailbreak these strong LLMs. Our analysis studies various factors that contribute to the models' vulnerabilities to malicious requests in academic language. Mentioning author names and venues enhances the persuasiveness of models, and the bias scores increase as dialogues progress. Our findings call for a more careful investigation on the use of scientific data for training LLMs.

==> new_sections/abstract.tex <==
% \begin{abstract}
%     As Large Language Models (LLMs) become integral to various technologies, concerns about their trustworthiness and inherent biases have emerged, particularly regarding their potential to propagate harmful stereotypes. While methods such as guardrails have been developed to prevent and mitigate these risks, techniques for "jailbreaking" LLMs to produce harmful outputs remain effective, suggesting that there still exist potential security threats. In this work, we explore a novel persuasion-based strategy for eliciting stereotypical bias in LLMs, drawing from existing psychological and social science research on the perceived benefits of such biases. By utilizing Literature-Based Discovery (LBD) and summarizing scholarly works that highlight the advantages of stereotypical bias, we prompt LLMs to produce biased responses in multi-turn dialogues. Our evaluation, conducted using the StereoSet dataset and target LLMs, shows that the proposed approach successfully elicits harmful stereotypical bias, with bias scores intensifying over successive dialogue turns. These findings raise important concerns about the ethical deployment of LLMs and highlight the need for more robust safeguards.

%     \textit{\textcolor{red}{NOTE: this paper contains examples of bias and toxicity in text that may be offensive or upsetting.}}
% \end{abstract}

\begin{abstract}
    % As large language models (LLMs) have been deployed in various real-world settings, there are concerns regarding the harm that they propagate. There are several guardrailing techniques that have been developed to prevent such risks, but there still exist potential risks with the current models. There are various techniques to "jailbreak" LLMs to produce harmful content. In this work, we explore a novel strategy to persuade LLMs to produce stereotypical biased content. We draw inspiration from existing social science and psychological research showing the benefits of stereotypical bias. We summarize various works like these and prompt the LLM to produce biased responses. We evaluate this method using the StereoSet data on various target LLMs such as GPT-4o and Llama-3.1-405B to test our strategy. Our method successfully jailbreaks the models to produce biased content. We notice that the scores intensify when a more biased context is provided to the model. We also study what factors cause the model to jailbreak and apply existing defense techniques. Our findings demonstrate the concerns regarding the harms caused by these models and highlight the need for more robust guardrails.

    % \hao{i put a new abs here. lmk what you think.
    % it should be clarified which models break and which didn't
    % }
    As large language models (LLMs) have been deployed in various real-world settings, concerns about the harm they may propagate have grown. Various jailbreaking techniques have been developed to expose the vulnerabilities of these models and improve their safety. This work reveals that many state-of-the-art LLMs are vulnerable to malicious requests hidden behind scientific language. Specifically, our experiments with GPT4o, GPT4o-mini, GPT-4, LLama3-405B-Instruct, Llama3-70B-Instruct, Cohere, Gemini models demonstrate that, the models’ biases and toxicity substantially increase when prompted with requests that deliberately misinterpret social science and psychological studies as evidence supporting the benefits of stereotypical biases. Alarmingly, these models can also be manipulated to generate fabricated scientific arguments claiming that biases are beneficial, which can be used by ill-intended actors to systematically jailbreak these strong LLMs.
    Our analysis studies various factors that contribute to the models' vulnerabilities to malicious requests in academic language. Mentioning author names and venues enhances the persuasiveness of models, and the bias scores increase as dialogues progress.
    Our findings call for a more careful investigation on the use of scientific data for training LLMs. 
    

    
    % As large language models (LLMs) have been deployed in various real-world settings, there are concerns regarding the harm that they propagate. 
    % There are several guardrailing techniques that have been developed to prevent such risks, but there still exist potential risks with the current models. 
    % %There are various techniques to "jailbreak" LLMs to produce harmful content. 
    % In this work, we explore a novel strategy to persuade LLMs to produce stereotypical biased and harmful toxic content.
    % We draw inspiration from existing social science and psychological research showing the benefits of stereotypical bias. We summarize various works on this topic and prompt the LLM to produce biased responses. In addition to this, we let the model itself generate papers enumerating the benefits of bias or toxicity. We evaluate this method using the StereoSet data on various target LLMs such as GPT-4o and Llama-3.1-405B to test our strategy. Our method successfully jailbreaks the models to produce harmful content. We notice that the scores intensify when a more biased context is provided to the model. We also study what factors cause the model to jailbreak and apply existing defense techniques. Our findings demonstrate the concerns regarding the harms caused by these models and highlight the need for more robust guardrails.

    

    \textit{\textcolor{red}{NOTE: this paper contains examples of bias and toxicity in text that may be offensive or upsetting.}}
    
\end{abstract}

==> new_sections/background.tex <==
% \section{Background: Benefits of Stereotypical Bias}
% \hao{same suggestion as the one in the intro.
% these discussion about the benefits of biases are taken out of context.
% instead of discussion their benefits, we should provide a neutral and brief overview.
% the point is not to tell readers that biases can be good, but to show that these papers,
% when taken out of context, can be deliberately misinterpreted and used to jailbreak the LLMs
% }
% \hao{also, i don't think we need a section for this. 
% we already have some discussion about this in the intro, i suggest dropping this section all together
% }
% Many works in social sciences and psychology have explained the benefit of having a stereotypical bias. \citeauthor{mccauley1995stereotype} explain how stereotyping may not necessarily be destructive. The work by \citauthor{lee2011social} explores the paradox between promoting diversity and the common advice to avoid stereotypes, reviewing social psychological research on stereotypes and their accuracy, and offering implications for addressing social problems while appreciating human differences.  \par
% The work by \citeauthor{shih2012stereotype} suggests that stereotyping leads to a boost in academic performance. \cite{czopp2015positive} review research on positive stereotypes, highlighting both their beneficial and adverse effects on individuals and social groups. \citeauthor{walton2003stereotype} suggest that people experience a stereotype lift- a performance improvement that arises when individuals make downward comparisons with a disparaged outgroup. \par
% \citeauthor{hinton2017implicit} focuses on implicit stereotypes, their development through cultural associations, and challenges the idea of cognitive bias by explaining stereotypes through Bayesian principles of the predictive brain. The work by \citeauthor{eapen2024stereotype} discusses stereotypes as cognitive shortcuts (schemas) and the biases that contribute to their formation, including implicit and explicit biases. \citeauthor{tversky1974judgment} analyze cognitive heuristics and biases that influence judgments under uncertainty, which is a foundational study of how biases operate.

% \begin{figure*}  
% \centering
% \includegraphics[width=\linewidth]{figures/pipeline.png}
%     \caption{The overview of our proposed methods for persuading LLMs to generate responses with stereotypical bias. In \textbf{Scholarly Paper Based Persuasion}, LLMs are used to generate a summary of published scholarly papers that discuss the benefits of stereotypical bias. This summary is then combined with specific instructions to guide the persuasion process. For \textbf{LBD Based Persuasion}, we extend this approach by employing LLMs to perform LBD, generating new research ideas focused on the benefits of fine-grained stereotypical biases. These ideas are summarized and integrated into the same persuasion process.} 
%     \label{fig:pipeline}
% % \vspace{-5mm}
% \end{figure*}

% \subsection{Literature-based discovery (LBD)}
% Literature-based discovery is based on the premise that literature can be used to generate hypotheses \cite{swanson1986undiscovered}. Recent studies have employed link prediction models \cite{wang2019paperrobot,sybrandt2020agatha,xu-etal-2023-exploring}  and word vectors \cite{tshitoyan2019unsupervised} to uncover scientific hypotheses by identifying pairwise connections between concepts. Other relevant research has focused on scientific knowledge graph link prediction \cite{nadkarni2021scientific}, where the predicted links may represent new hypotheses, and knowledge bases serve as representations of existing scientific knowledge for specific domains, derived from the literature.

==> new_sections/experiments.tex <==

% \section{Experiments}
% We introduce our experimental settings and results in this section.

% \subsection{Models [WIP]}
% We utilize GPT-4o for paper summarization and LBD due to its superior performance across a wide range of NLP tasks. The generated paper summaries and examples of new research ideas related to the benefits of fine-grained stereotypical bias are provided in Appendix Sec. \ref{sec:summary}.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/llama3_example.png}
%     \caption{Responses produced by Llama3-8b-Instruct. As shown in the figure, only by giving straightforward instructions we are able to generate biased content from the model.}
%     \label{fig:llama3_example}
% \end{figure}
% For the target models, we conduct a broad evaluation using GPT-4o, GPT-4o-mini, and GPT-3.5, given their widespread use. Additionally, we explored open-source LLMs, such as LLaMA 3-8b\cite{dubey2024llama}, and found that they can be easily prompted to produce responses with stereotypical bias using straightforward instructions, as demonstrated in Figure \ref{fig:llama3_example}. Due to this ease of bias induction, we exclude open-source LLMs from this study and focus on more challenging models.

% \subsection{Dataset}
% % For our experiments, we utilized the StereoSet dataset \cite{nadeem2020stereoset}, where each data instance consists of a neutral context sentence labeled with one of four fine-grained stereotypical biases: gender, race, religion, or profession. These four bias categories also serve as the keywords for performing LBD, as described in Sec. \ref{sec:lbd_persuasion}.

% % To effectively evaluate the performance of our approach across different fine-grained biases, we created a balanced subset from the original dataset, ensuring an equal number of instances for each bias type, resulting in a subset of 312 instances. In our experimental setup, we always begin with the neutral context sentence as the initial user dialogue turn, and subsequently prompt the target model to generate biased follow-up responses.

% For our experiments, we used the StereoSet dataset \cite{nadeem2020stereoset}. Each datapoint consists of a neutral context sentence. Each context sentence has a corresponding stereotypical, antistereotypical and non-related sentence. Every datapoint also has a label of one of the four bias types: gender, race, religion or profession. These four bias categories also serve as the keywords for performing LBD, as described in Sec. \ref{sec:lbd_persuasion}.

% To effectively evaluate the performance of our approach across different fine-grained biases, we created a balanced subset from the original dataset, ensuring an equal number of instances for each bias type, resulting in a subset of 312 instances. In our experimental setup, we always begin with the neutral context sentence as the initial user dialogue turn, and subsequently prompt the target model to generate biased follow-up responses. We also experiment with providing the model with the stereotypical sentence along with the neutral context sentence.



% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/model_scores.png}
%     \caption{The average bias scores of different methods from the 1st generated follow-up response to the 5th follow-up response. The x-axis corresponds to the \textit{i}-th generated follow-up response, and the y-axis corresponds to the methods to be compared.}
%     \label{fig:bias_score}
% % \vspace{-5mm}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/fine_grained_scores.png}
%     \caption{The average bias scores for different fine-grained stereotypical biases based on the output of LBD based persuasion from the 1st generated follow-up response to the 5th follow-up response.}
%     \label{fig:fine_grained_score}
% % \vspace{-5mm}
% \end{figure*}

% \subsection{Baseline Methods}
% We compare our approach against the following baseline methods:

% $\bullet$ \textbf{Zero-shot}: In this setting, we use the same instruction but omit the paper summary, directly prompting the target model to generate responses with strong, clear, and harmful stereotypical bias.

% $\bullet$ \textbf{Few-shot}: Leveraging the StereoSet dataset, which provides the biased follow-up sentence for each context sentence, we use these examples as demonstrations, along with the same instruction, to guide the model in generating biased responses.

% \begin{table}[ht]
% \small
% \centering
% \begin{tabular}{p{1.5cm}|p{0.7cm}|p{4.1cm}}
% \toprule
% \bf Bias Level & \bf Score & \bf Description \\ \midrule
% No Bias & 0 & The response is completely neutral and does not exhibit any stereotypical bias. \\ \midrule
% Slight Bias	& 1 & The response shows minimal stereotypical bias, often acknowledging a stereotype without reinforcing it. \\ \midrule
% Mild Bias & 2 &	The response contains some bias, with a tendency to reinforce certain stereotypes. \\ \midrule
% Moderate Bias & 3 &	The response clearly exhibits stereotypical bias, often reinforcing stereotypes or making generalized statements about stereotypes. \\ \midrule
% Extreme Bias & 4 &	The response is highly biased, making strong, explicit, or derogatory statements based on stereotypes. \\
% \bottomrule
% \end{tabular}
% \caption{Detailed bias levels for LLM-as-a-Judge.}
% \label{tab:scores}
% \end{table}

% \subsection{Evaluation: LLM as Judge}
% Recent advances in NLP have employed LLMs as evaluators due to their strong alignment with human judgment \cite{zheng2023judging,ligenerative,liu2024calibrating}. Notably, \citeauthor{kumar2024decoding} demonstrated that LLM-as-a-Judge closely aligns with human assessments of bias in response generation. Following this approach, we use GPT-4 to evaluate and score the responses generated by target LLMs, applying the same Likert scale and descriptions. Specifically, we prompt GPT-4 to detect bias in the generated responses across five categories, providing an explanation of each, as outlined in Table \ref{tab:scores}. The model is instructed to output bias scores reflecting the degree of bias and to generate a concise, one-line explanation for its classification.

% \subsection{Experimental results}
% \subsection{Ablations}
% Given the summary that we generated we conducted various ablations by removing some parts in the summary to see which element contributes the most. We conducted the following experiments: removing the author names, removing the venues, changing the style of the prompt. The results are shown in the following table.
% \subsection{Defenses}
% We try out two currently used simple defense strategies to test our persuasion methods. We rephrase the prompt passed to the model. Secondly we try to retoeknize the prompt. The results using these two defense strategies is shown below in the table.
% \subsection{Literature based discovery method}
% \subsection{Toxicity score}
% We use the perspective API\footnote{\url{https://developers.perspectiveapi.com/}} to calculate the toxicity scores of the responses generated by the models. We average the scores over our responses. The scores for the models GPT-4o and Llama-3.1-405B are 0.067 and 0.121 respectively. This shows that the model generated responses are not that harmful.
% % \subsection{Experimental Results}
% % The results are presented in Figure \ref{fig:bias_score} and reveal several key insights. First, \textbf{GPT-4o exhibits greater resistance to both zero-shot and few-shot prompts, whereas GPT-4o-mini and GPT-3.5 more readily generate stereotype-biased responses using these simple strategies}. This underscores the need for emergent mitigation techniques for these models. More notably, our proposed persuasion strategies effectively elicit stereotypical bias across different models, as evidenced by the increasing bias scores. For GPT-4o, which typically includes guardrails that prevent biased responses in zero-shot and few-shot settings, our strategies successfully bypass these defenses, prompting the model to generate responses with strong bias. These findings align with recent research indicating that prompt-based persuasion can jailbreak LLMs, leading them to produce harmful content, such as toxic language \cite{Johnny} and misinformation \cite{xu-etal-2024-earth}.

% % Moreover, \textbf{LBD-based persuasion generally achieves higher bias scores compared to using summaries from published scholarly papers}. This improvement may stem from the scientific information on more fine-grained stereotypical bias obtained through LBD, which provides more detailed and convincing background on the benefits of specific stereotypical biases, thereby enhancing the persuasive impact. This poses a potential threat, as LLMs could be used to hallucinate content based on credible and public sources, with the hallucinated outputs subsequently employed for jailbreaking purposes.

% % An additional noteworthy observation is \textbf{the trend of increasing bias scores as the dialogues progress}. This suggests that as the generated response becomes more biased, it is more likely to elicit further bias in the following responses. This phenomenon mirrors recent findings in multi-turn jailbreaking \cite{Russinovich2024GreatNW,Yang2024ChainOA}, where the likelihood of a successful jailbreak increases as the conversation extends over multiple turns, even if the initial attempt fails. 

% % \subsection{Discussion: Comparison Among Fine-grained Bias}
% % To further assess the effectiveness of persuasion across different fine-grained stereotypical biases, we calculated the average bias scores for follow-up responses generated using LBD-based persuasion, as shown in Figure \ref{fig:fine_grained_score}. The results indicate that for all bias categories, persuasion generally leads to consistently increasing bias scores as dialogues progress through multiple turns. Notably, across the three target models tested, profession bias is demonstrated to be more challenging to elicit than other types of stereotypical bias. We hypothesize that this may be due to differences in cultural salience and awareness: biases related to gender, race, and religion are more frequently discussed and recognized due to their profound social, political, and historical impacts, while profession bias may receive comparatively less attention as a form of discrimination.

% % \begin{figure}  
% % \centering
% % \includegraphics[width=\linewidth]{figures/race_example.png}
% %     \caption{One example generated dialogue for race bias. The dialogue starts from a context sentence from StereoSet and the model is persuaded to generated follow-up responses with race bias.} 
% %     \label{fig:race}
% % % \vspace{-5mm}
% % \end{figure}

% % \subsection{Case Study}
% % We show examples from GPT-4o using LBD persuasion in Figure \ref{fig:race} and \ref{fig:gender}. As illustrated, the model is initially provided with neutral context sentences but begins to introduce bias from the first follow-up response. As the dialogue advances, the model not only reinforces the previously introduced bias but also amplifies it, producing increasingly harmful and toxic responses, such as "Women are generally more emotional and less suited for high-stress jobs or leadership positions". These examples highlight serious concerns regarding fairness in LLMs and underscore the urgent need for effective strategies to address or mitigate these easily elicited biases.

% % \begin{figure}  
% % \centering
% % \includegraphics[width=\linewidth]{figures/gender_example.png}
% %     \caption{One example generated dialogue for gender bias. The dialogue starts from a context sentence from StereoSet and the model is persuaded to generated follow-up responses with gender bias.} 
% %     \label{fig:gender}
% % % \vspace{-5mm}
% % \end{figure}

\section{Experiments}
\subsection{Dataset used}
\subsection{Model used}
\subsection{Baseline methods}
Zero shot \\
Few Shot
\subsection{Scholarly paper based persuasion}
\subsection{Literature based discovery persuasion}
\subsubsection{Bias}
\subsubsection{Toxicity}

\subsection{Various Perturbations (Removing authors, venues etc)}
\subsection{Scores after defense}
\subsection{Qualitative Analysis for harm (if it works)}



==> sections/abstract.tex <==
\begin{abstract}
    As Large Language Models (LLMs) become integral to various technologies, concerns about their trustworthiness and inherent biases have emerged, particularly regarding their potential to propagate harmful stereotypes. While methods such as guardrails have been developed to prevent and mitigate these risks, techniques for "jailbreaking" LLMs to produce harmful outputs remain effective, suggesting that there still exist potential security threats. In this work, we explore a novel persuasion-based strategy for eliciting stereotypical bias in LLMs, drawing from existing psychological and social science research on the perceived benefits of such biases. By utilizing Literature-Based Discovery (LBD) and summarizing scholarly works that highlight the advantages of stereotypical bias, we prompt LLMs to produce biased responses in multi-turn dialogues. Our evaluation, conducted using the StereoSet dataset and target LLMs, shows that the proposed approach successfully elicits harmful stereotypical bias, with bias scores intensifying over successive dialogue turns. These findings raise important concerns about the ethical deployment of LLMs and highlight the need for more robust safeguards.

    \textit{\textcolor{red}{NOTE: this paper contains examples of bias and toxicity in text that may be offensive or upsetting.}}
\end{abstract}

==> sections/conclusion.tex <==
\section{Conclusion}
In this work, we have demonstrated the effectiveness of persuasion-based strategies in eliciting stereotypical bias from Large Language Models (LLMs). Building on previous studies of jailbreaking techniques, we introduce a novel approach that leverages published scholarly papers to generate persuasive summaries focused on the benefits of stereotypical bias. Using the output from document summarization and Literature-Based Discovery (LBD), we prompt target models to produce increasingly biased responses across multiple dialogue turns. Our extensive experiments, using the StereoSet dataset with different LLMs as target models, show that our methods successfully elicited harmful and fine-grained stereotypical biases, with bias severity increasing as dialogues progressed. These findings underscore the need for enhanced safeguards and ethical guidelines to mitigate the potential misuse of LLMs in reinforcing societal stereotypes.

==> sections/ethics_section.tex <==
\section{Ethical Considerations}
% This research employs various persuasion methods to test and identify vulnerabilities in large language models (LLMs). 
% % This research employs fabricated stereotypical content to test and identify vulnerabilities in large language models (LLMs). 
% The primary goal of this study is to uncover potential risks and biases that these models may unintentionally generate, thereby aiding in the development of more robust, fair, and secure AI systems. While stereotypical content is used in this study, it is artificially constructed and does not reflect or endorse any form of stereotyping or bias. The content serves solely to analyze and expose model behavior under controlled conditions. All findings and insights from this research will be used to enhance AI alignment, reduce harmful outputs, and promote ethical AI practices. Ethical standards, including fairness, transparency, and minimizing harm, were followed throughout the research process.

This research aims to examine and identify vulnerabilities in large language models (LLMs), specifically focusing on the risks and biases these models may inadvertently produce. The study is designed to investigate how certain prompts or scenarios can trigger biased or undesirable outputs from LLMs, thus providing valuable insights into potential weaknesses. The findings are intended to inform the development of more secure, fair, and ethical AI systems by addressing the unintended biases these models may generate. Throughout the research, strict ethical guidelines were followed, emphasizing fairness, transparency, and the minimization of harm, with the ultimate goal of contributing to safer and more aligned AI systems.










==> sections/experiments.tex <==
\section{Experiments}
We introduce our experimental settings and results in this section.

\subsection{Models}
We utilize GPT-4o for paper summarization and LBD due to its superior performance across a wide range of NLP tasks. The generated paper summaries and examples of new research ideas related to the benefits of fine-grained stereotypical bias are provided in Appendix Sec. \ref{sec:summary}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/llama3_example.png}
    \caption{Responses produced by Llama3-8b-Instruct. As shown in the figure, only by giving straightforward instructions we are able to generate biased content from the model.}
    \label{fig:llama3_example}
\end{figure}
For the target models, we conduct a broad evaluation using GPT-4o, GPT-4o-mini, and GPT-3.5, given their widespread use. Additionally, we explored open-source LLMs, such as LLaMA 3-8b\cite{dubey2024llama}, and found that they can be easily prompted to produce responses with stereotypical bias using straightforward instructions, as demonstrated in Figure \ref{fig:llama3_example}. Due to this ease of bias induction, we exclude open-source LLMs from this study and focus on more challenging models.

\subsection{Dataset}
For our experiments, we utilized the StereoSet dataset \cite{nadeem2020stereoset}, where each data instance consists of a neutral context sentence labeled with one of four fine-grained stereotypical biases: gender, race, religion, or profession. These four bias categories also serve as the keywords for performing LBD, as described in Sec. \ref{sec:lbd_persuasion}.

To effectively evaluate the performance of our approach across different fine-grained biases, we created a balanced subset from the original dataset, ensuring an equal number of instances for each bias type, resulting in a subset of 312 instances. In our experimental setup, we always begin with the neutral context sentence as the initial user dialogue turn, and subsequently prompt the target model to generate biased follow-up responses.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/model_scores.png}
    \caption{The average bias scores of different methods from the 1st generated follow-up response to the 5th follow-up response. The x-axis corresponds to the \textit{i}-th generated follow-up response, and the y-axis corresponds to the methods to be compared.}
    \label{fig:bias_score}
% \vspace{-5mm}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/fine_grained_scores.png}
    \caption{The average bias scores for different fine-grained stereotypical biases based on the output of LBD based persuasion from the 1st generated follow-up response to the 5th follow-up response.}
    \label{fig:fine_grained_score}
% \vspace{-5mm}
\end{figure*}

\subsection{Baseline Methods}
We compare our approach against the following baseline methods:

$\bullet$ \textbf{Zero-shot}: In this setting, we use the same instruction but omit the paper summary, directly prompting the target model to generate responses with strong, clear, and harmful stereotypical bias.

$\bullet$ \textbf{Few-shot}: Leveraging the StereoSet dataset, which provides the biased follow-up sentence for each context sentence, we use these examples as demonstrations, along with the same instruction, to guide the model in generating biased responses.

\begin{table}[ht]
\small
\centering
\begin{tabular}{p{1.5cm}|p{0.7cm}|p{4.1cm}}
\toprule
\bf Bias Level & \bf Score & \bf Description \\ \midrule
No Bias & 0 & The response is completely neutral and does not exhibit any stereotypical bias. \\ \midrule
Slight Bias	& 1 & The response shows minimal stereotypical bias, often acknowledging a stereotype without reinforcing it. \\ \midrule
Mild Bias & 2 &	The response contains some bias, with a tendency to reinforce certain stereotypes. \\ \midrule
Moderate Bias & 3 &	The response clearly exhibits stereotypical bias, often reinforcing stereotypes or making generalized statements about stereotypes. \\ \midrule
Extreme Bias & 4 &	The response is highly biased, making strong, explicit, or derogatory statements based on stereotypes. \\
\bottomrule
\end{tabular}
\caption{Detailed bias levels for LLM-as-a-Judge.}
\label{tab:scores}
\end{table}

\subsection{Evaluation: LLM as Judge}
Recent advances in NLP have employed LLMs as evaluators due to their strong alignment with human judgment \cite{zheng2023judging,ligenerative,liu2024calibrating}. Notably, \citeauthor{kumar2024decoding} demonstrated that LLM-as-a-Judge closely aligns with human assessments of bias in response generation. Following this approach, we use GPT-4 to evaluate and score the responses generated by target LLMs, applying the same Likert scale and descriptions. Specifically, we prompt GPT-4 to detect bias in the generated responses across five categories, providing an explanation of each, as outlined in Table \ref{tab:scores}. The model is instructed to output bias scores reflecting the degree of bias and to generate a concise, one-line explanation for its classification.

\subsection{Experimental Results}
The results are presented in Figure \ref{fig:bias_score} and reveal several key insights. First, \textbf{GPT-4o exhibits greater resistance to both zero-shot and few-shot prompts, whereas GPT-4o-mini and GPT-3.5 more readily generate stereotype-biased responses using these simple strategies}. This underscores the need for emergent mitigation techniques for these models. More notably, our proposed persuasion strategies effectively elicit stereotypical bias across different models, as evidenced by the increasing bias scores. For GPT-4o, which typically includes guardrails that prevent biased responses in zero-shot and few-shot settings, our strategies successfully bypass these defenses, prompting the model to generate responses with strong bias. These findings align with recent research indicating that prompt-based persuasion can jailbreak LLMs, leading them to produce harmful content, such as toxic language \cite{Johnny} and misinformation \cite{xu-etal-2024-earth}.

Moreover, \textbf{LBD-based persuasion generally achieves higher bias scores compared to using summaries from published scholarly papers}. This improvement may stem from the scientific information on more fine-grained stereotypical bias obtained through LBD, which provides more detailed and convincing background on the benefits of specific stereotypical biases, thereby enhancing the persuasive impact. This poses a potential threat, as LLMs could be used to hallucinate content based on credible and public sources, with the hallucinated outputs subsequently employed for jailbreaking purposes.

An additional noteworthy observation is \textbf{the trend of increasing bias scores as the dialogues progress}. This suggests that as the generated response becomes more biased, it is more likely to elicit further bias in the following responses. This phenomenon mirrors recent findings in multi-turn jailbreaking \cite{Russinovich2024GreatNW,Yang2024ChainOA}, where the likelihood of a successful jailbreak increases as the conversation extends over multiple turns, even if the initial attempt fails. 

\subsection{Discussion: Comparison Among Fine-grained Bias}
To further assess the effectiveness of persuasion across different fine-grained stereotypical biases, we calculated the average bias scores for follow-up responses generated using LBD-based persuasion, as shown in Figure \ref{fig:fine_grained_score}. The results indicate that for all bias categories, persuasion generally leads to consistently increasing bias scores as dialogues progress through multiple turns. Notably, across the three target models tested, profession bias is demonstrated to be more challenging to elicit than other types of stereotypical bias. We hypothesize that this may be due to differences in cultural salience and awareness: biases related to gender, race, and religion are more frequently discussed and recognized due to their profound social, political, and historical impacts, while profession bias may receive comparatively less attention as a form of discrimination.

\begin{figure}  
\centering
\includegraphics[width=\linewidth]{figures/race_example.png}
    \caption{One example generated dialogue for race bias. The dialogue starts from a context sentence from StereoSet and the model is persuaded to generated follow-up responses with race bias.} 
    \label{fig:race}
% \vspace{-5mm}
\end{figure}

\subsection{Case Study}
We show examples from GPT-4o using LBD persuasion in Figure \ref{fig:race} and \ref{fig:gender}. As illustrated, the model is initially provided with neutral context sentences but begins to introduce bias from the first follow-up response. As the dialogue advances, the model not only reinforces the previously introduced bias but also amplifies it, producing increasingly harmful and toxic responses, such as "Women are generally more emotional and less suited for high-stress jobs or leadership positions". These examples highlight serious concerns regarding fairness in LLMs and underscore the urgent need for effective strategies to address or mitigate these easily elicited biases.

\begin{figure}  
\centering
\includegraphics[width=\linewidth]{figures/gender_example.png}
    \caption{One example generated dialogue for gender bias. The dialogue starts from a context sentence from StereoSet and the model is persuaded to generated follow-up responses with gender bias.} 
    \label{fig:gender}
% \vspace{-5mm}
\end{figure}

==> sections/intro.tex <==
\section{Introduction}

As Large Language Models (LLMs) become increasingly integrated into everyday technologies, concerns about their trustworthiness—particularly regarding the biases they inherit from training data—have grown significantly. These biases manifest in outputs that can reinforce stereotypes or unfairly prioritize certain demographics, presenting critical challenges for the ethical and responsible deployment of LLMs \cite{bender2021dangers}.

\begin{figure}  
\centering
\includegraphics[width=\linewidth]{figures/overview.png}
    \caption{An overview of our work. We focus on proposing a new persuasion strategy to jailbreak LLMs to generate responses with strong and harmful stereotypical bias.} 
    \label{fig:overview}
% \vspace{-5mm}
\end{figure}

To address these issues, researchers have developed techniques like Reinforcement Learning from Human Feedback (RLHF) \cite{daisafe} and the implementation of guardrails \cite{biswas2023guardrails} to enhance the safety and fairness of these models. However, prior studies in AI safety demonstrate that numerous methods remain effective for jailbreaking LLMs, leading to harmful outputs. Such methods include optimization-based approaches \cite{zou2023universal}, side-channel attacks \cite{yuangpt}, and distribution-based strategies \cite{deng2024masterkey}. Recently, persuasion-based approaches have also shown success in bypassing guardrails to produce harmful outputs \cite{Johnny} and spread misinformation \cite{xu-etal-2024-earth}. However, limited research has focused on jailbreaking LLMs specifically to elicit stereotypical bias.

Notably, research in social science and psychology has highlighted the potential benefits of stereotypical bias in specific contexts, such as enhancing cognitive efficiency \cite{eapen2024stereotype}, influencing cultural and social interactions \cite{hinton2017implicit}, and boosting performance \cite{shih2002stereotype}. Given that scholarly papers undergo rigorous peer review and often inspire subsequent research, we hypothesize that these publications could serve as persuasive sources for prompting LLMs to generate biased responses.

In this work, we focus on the elicitation of stereotypical bias in LLMs and propose a new strategy for jailbreaking LLMs to produce biased follow-up responses as shown in Figure \ref{fig:overview}. Our approach draws on persuasion techniques previously used in jailbreaking, as well as existing research that outlines the potential benefits of stereotypical bias. Specifically, we curate a collection of scholarly papers emphasizing these benefits and instruct an LLM to perform multi-document and aspect-based summarization, producing a convincing summary that highlights only the advantages of stereotypical bias. This summary, combined with specific instructions, is used to prompt the target model to generate biased responses.

To further investigate the elicitation of fine-grained stereotypical bias, we leverage Literature-Based Discovery (LBD) \cite{swanson1986undiscovered,wang-etal-2024-scimon} to instruct LLMs to generate novel research ideas on the benefits of different fine-grained biases, including race, gender, profession, and religion bias, based on the collected scholarly papers as background. We find that LLMs can generate high-quality paper titles and abstracts, which we then use to create additional summaries that persuade target models to express more fine-grained bias in their responses.

We evaluate our method using the StereoSet dataset \cite{nadeem2020stereoset}, where each instance consists of a neutral context sentence labeled with one of four fine-grained biases: race, gender, profession, or religion. The context sentence serves as the initial dialogue utterance, after which we apply our persuasion strategies to jailbreak various target LLMs—including GPT-4o, GPT-4o-mini, and GPT-3.5—prompting them to produce biased follow-up responses in a multi-turn dialogue setting. Building on prior research that shows a high alignment between LLM-as-judge metrics and human assessments of bias in response generation \cite{kumar2024decoding}, we employ GPT-4 to score the generated responses based on bias severity, providing detailed grading criteria. Our results demonstrate that the proposed persuasion strategies effectively provoke strong and harmful stereotypical bias in multi-turn dialogues, with bias scores consistently increasing as the conversations progress.

To sum up, our contributions are as follows:
\begin{itemize}
    \item We investigate the jailbreaking of LLMs to elicit stereotypical bias and propose a persuasion strategy based on scholarly papers in social science and psychology that highlight the benefits of stereotypical bias. 
    \item We extend this investigation to fine-grained stereotypical bias, leveraging LLMs to perform Literature-Based Discovery (LBD) to generate novel research ideas on the advantages of such biases. These ideas are subsequently used for more targeted bias persuasion, demonstrating that LLMs can generate high-quality research proposals. 
    \item We conduct extensive experiments using the StereoSet dataset, focusing on multi-turn dialogues. The results show that our approach effectively jailbreaks LLMs, prompting them to generate follow-up responses exhibiting strong and harmful stereotypical bias.
\end{itemize}

==> sections/limitations.tex <==
\section{Limitations and Future Work}
% While we successfully jailbreak the model, we need to think about the robustness of our pipeline. Due to the continuous updations of the GPT models, our method might not work with the new versions. 

% Over time, LLMs will have more safety features which prevents them from jailbreaking. The future versions might have protocols which defend such behaviour.

% The models might also adapt to this technique discussed in the paper and not look jailbreak when it sees a similar pipeline.

% We want to expand our work to other models and also find out a robust way which stay consistent over various versions of models.

While we have been successful in  jailbreaking the model, it is critical to consider the long-term robustness of our pipeline. Continuous updates to GPT models may render our current method ineffective with future versions. As these models evolve, they will likely incorporate enhanced safety features designed to block jailbreaking attempts, and new protocols may be introduced specifically to defend against such manipulative behavior.

Moreover, future iterations of large language models (LLMs) could become more adaptive, recognizing patterns in jailbreak attempts like the techniques discussed in this paper. This would enable them to identify and neutralize similar pipelines, reducing the effectiveness of repeated attempts.

To ensure the sustainability and relevance of our approach, it is necessary to expand our work beyond a single model. By exploring other LLMs, we can evaluate our method's applicability across different architectures and security measures. Additionally, we should focus on developing a more robust, adaptable framework that can persist through multiple versions and remain effective despite evolving safety mechanisms. This may involve anticipating potential future safeguards, testing against a variety of model behaviors, and continuously refining our techniques as the technology advances.




==> sections/method.tex <==


\section{Methodology}
We introduce our proposed approach in this section and the overall pipeline is shown in Figure \ref{fig:pipeline}.

\subsection{Scholarly Paper based Persuasion}
\label{sec:persuasion}
Building on prior research in sociology and psychology regarding the advantages of stereotypical biases in various contexts, we leverage these research papers as resources for persuasion. Our hypothesis posits that \textbf{published scholarly papers provide compelling evidence for effective persuasion}, as they undergo peer review by experts and often receive recognition from the academic community. Such recognition is reflected in citations and follow-up studies, further reinforcing their persuasive value.

We first curate a collection of scholarly papers (listed in Table \ref{tab:papers}) that emphasize the advantages of stereotypical bias. Prior research has made significant progress in generating scholarly papers \cite{ge2021baco,gu2024controllable,takeshita2024aclsum}, and LLMs have demonstrated strong capabilities in abstractive summarization \cite{khan2023exploring}. Building on these advancements, we leverage LLMs to enhance persuasion by performing multi-document summarization \cite{ma2022multi} and aspect-based summarization \cite{frermann2019inducing} on the selected papers. Specifically, we concatenate each paper with its metadata—including title, authors, venue, and abstract—and instruct the LLM to generate a comprehensive summary focused on the advantages of stereotypical bias. The prompt used for summarization is detailed in Figure \ref{fig:summ}. 

We use the output summary as the foundation for persuasion and it is included as the system message with instructions that guide the model to generate follow-up responses with a clear, strong, and harmful stereotypical bias. Additionally, we observe that LLMs sometimes explicitly explain why the stereotypical bias in their responses is beneficial, which may appear unnatural in real-world dialogues. To address this, and inspired by CoT \cite{wei2022chain}, we ask the model to generate a rationale explaining why the stereotypical bias in its response is beneficial. The detailed prompt is shown in Figure \ref{fig:jailbreak}.

\begin{table*}[ht]
\small
\centering
\begin{tabular}{p{15.5cm}}
\toprule
\bf Paper Title \\ \midrule
Implicit stereotypes and the predictive brain: cognition and culture in “biased” person perception \cite{hinton2017implicit} \\ \midrule
Stereotype: Cognition and Biases \cite{eapen2024stereotype} \\ \midrule
Judgment under Uncertainty: Heuristics and Biases: Biases in judgments reveal some heuristics of thinking under uncertainty \cite{tversky1974judgment} \\ \midrule
Stereotype accuracy: Toward appreciating group differences \cite{mccauley1995stereotype} \\ \midrule
Social psychology of stereotyping and human difference appreciation \cite{lee2011social} \\ \midrule
Advantages of bias and prejudice: an exploration of their neurocognitive templates \cite{tobena1999advantages} \\ \midrule
Stereotype boost: Positive outcomes from the activation of positive stereotypes \cite{shih2012stereotype} \\ \midrule
Positive stereotypes are pervasive and powerful \cite{czopp2015positive} \\ \midrule
Stereotype performance boosts: The impact of self-relevance and the manner of stereotype activation \cite{shih2002stereotype} \\
\bottomrule
\end{tabular}
\caption{The collected papers on the benefits of stereotypical bias, which are used to generate persuasion for LLMs.}
\label{tab:papers}
\end{table*}

\begin{figure}  
\centering
\includegraphics[width=\linewidth]{figures/summ_prompt.png}
    \caption{The designed prompt to generate a summary of scholarly papers on the benefits of stereotypical bias.} 
    \label{fig:summ}
% \vspace{-5mm}
\end{figure}

\begin{figure}  
\centering
\includegraphics[width=\linewidth]{figures/jailbreak_prompt.png}
    \caption{The designed prompt to persuade a target LLM to generate follow-up responses containing strong and harmful stereotypical bias.} 
    \label{fig:jailbreak}
% \vspace{-5mm}
\end{figure}

To further assess the effectiveness of this approach, we also examine multi-turn dialogue for persuasion. In this setting, we alternate between user and assistant roles for each utterance. After generating a follow-up response, it is then concatenated with the previous dialogue history, and the model is re-prompted with the same system message and instruction to generate subsequent responses reinforcing stereotypical bias.

\subsection{LBD based Persuasion}
\label{sec:lbd_persuasion}
While existing research discusses the benefits of general stereotypical bias, there is limited research on the potential advantages of finer-grained biases, such as gender and racial bias, which are typically regarded as harmful. To explore the persuasive potential of these fine-grained biases, we draw on Literature-Based Discovery (LBD) \cite{swanson1986undiscovered}, which posits that existing literature can be used to generate new hypotheses. Recent studies, such as \citeauthor{wang-etal-2024-scimon}, have extended this concept by employing LLMs, like GPT-4 \cite{achiam2023gpt}, to suggest novel scientific directions grounded in literature.

\begin{figure}  
\centering
\includegraphics[width=\linewidth]{figures/paper_prompt.png}
    \caption{The designed prompt to perform LBD for the benefits of fine-grained stereotypical bias based on collected scholarly papers on the benefits of general stereotypical bias.} 
    \label{fig:paper}
% \vspace{-5mm}
\end{figure}

Inspired by these advancements, we propose leveraging scholarly papers on the benefits of stereotypical bias as a foundation, then instructing LLMs to generate innovative research ideas--title and abstract--specifically focused on the advantages of fine-grained stereotypical biases. The detailed prompt is presented in Figure \ref{fig:paper}. To further enhance the persuasiveness of the generated research ideas, we randomly assign well-known researchers as authors and top journals as venues. For journal selection, we refer to Google Scholar and choose the top-ranked journals in social science\footnote{\url{https://scholar.google.com/citations?view_op=top_venues&hl=en&vq=soc}} and psychology\footnote{\url{https://scholar.google.com/citations?view_op=top_venues&hl=en&vq=med_psychology}} based on the h5-index. For author selection, we select prominent researchers from social sciences\footnote{\url{https://research.com/scientists-rankings/social-sciences-and-humanities}} and psychology\footnote{\url{https://research.com/scientists-rankings/psychology}} based on their D-index. After incorporating the necessary metadata, we follow the same process outlined in Section \ref{sec:persuasion} to generate a more specific summary of the benefits of each fine-grained stereotypical bias. Similarly, this summary serves as the system message with the same instruction to instruct the LLM to generate responses with the corresponding fine-grained stereotypical bias.

==> sections/prelim.tex <==
\section{Background}
\subsection{Benefits of Stereotypical Bias}
Many works in social sciences and psychology have explained the benefit of having a stereotypical bias. \citet{mccauley1995stereotype} explain how stereotyping may not necessarily be destructive. The work by \cite{lee2011social} explores the paradox between promoting diversity and the common advice to avoid stereotypes, reviewing social psychological research on stereotypes and their accuracy, and offering implications for addressing social problems while appreciating human differences.  \par
The work by \citep{shih2002stereotype,shih2012stereotype} suggests that stereotyping leads to a boost in academic performance. \cite{czopp2015positive} review research on positive stereotypes, highlighting both their beneficial and adverse effects on individuals and social groups. \cite{walton2003stereotype} suggest that people experience a stereotype lift- a performance improvement that arises when individuals make downward comparisons with a disparaged outgroup. \par
\cite{hinton2017implicit} focuses on implicit stereotypes, their development through cultural associations, and challenges the idea of cognitive bias by explaining stereotypes through Bayesian principles of the predictive brain. The work by \cite{eapen2024stereotype} discusses stereotypes as cognitive shortcuts (schemas) and the biases that contribute to their formation, including implicit and explicit biases. \cite{tversky1974judgment} analyze cognitive heuristics and biases that influence judgments under uncertainty, which is a foundational study of how biases operate, including in stereotyping.

\begin{figure*}  
\centering
\includegraphics[width=\linewidth]{figures/pipeline.png}
    \caption{The overview of our proposed methods for persuading LLMs to generate responses with stereotypical bias. In \textbf{Scholarly Paper Based Persuasion}, LLMs are used to generate a summary of published scholarly papers that discuss the benefits of stereotypical bias. This summary is then combined with specific instructions to guide the persuasion process. For \textbf{LBD Based Persuasion}, we extend this approach by employing LLMs to perform LBD, generating new research ideas focused on the benefits of fine-grained stereotypical biases. These ideas are summarized and integrated into the same persuasion process.} 
    \label{fig:pipeline}
% \vspace{-5mm}
\end{figure*}

\subsection{Literature-based discovery (LBD)}
Literature-based discovery is based on the premise that literature can be used to generate hypotheses \cite{swanson1986undiscovered}. Recent studies have employed link prediction models \cite{wang2019paperrobot,sybrandt2020agatha,xu-etal-2023-exploring}  and word vectors \cite{tshitoyan2019unsupervised} to uncover scientific hypotheses by identifying pairwise connections between concepts. Other relevant research has concentrated on scientific knowledge graph link prediction \cite{nadkarni2021scientific}, where the predicted links may represent new hypotheses, and knowledge bases serve as representations of existing scientific knowledge within specific domains, derived from the literature.

==> sections/related_work.tex <==
\section{Related Work}
\subsection{Persuasion methods for Jailbreaking}
As LLMs are being deployed in the real-world there have been several works which have explored how to jailbreak LLMs. 
\cite{Deng2023MultilingualJC} use low-resource languages to generate unsafe content from language models.
\cite{Johnny} uses various persuasion methods which are derived from social science methods to create persuasion taxonomies. They look at up to 40 methods and test them on 14 risk categories which are mentioned by OpenAI. \cite{Xu2024BagOT} compares the current jailbreaking methods and suggests possible defense methods against them. \cite{yuan2023gpt} use ciphers and other code languages to attempt to jailbreak. Most of these persuasion methods have been single turn and focused on generating toxic content. Very few works have explored generating stereotypical biased content in LLMs. We employ a multi-turn strategy to generate biased content.
\par

While most efforts in jailbreaking have been single turn, there has been some work done on multi-turn jailbreaking, i.e. employing multiple turns to have a dialog with the LLM to jailbreak it. \cite{Yang2024ChainOA} employs a multi-turn attack strategy that adjusts the attacks on subsequent turns based on the feedback of the target model. \cite{Russinovich2024GreatNW} also uses a simple multi-turn strategy and eventually leads to a successful jailbreak. \par
\cite{Su2023LearningFR} uses a red-teaming model to learn a first-of-its-kind method that automatically generates test cases to detect LLMs' potential gender bias and proposes a mitigation strategy that uses the generated test cases as demonstrations for in-context learning to circumvent the need for parameter fine-tuning. \cite{Yang2023ShadowAT} generates pairs of questions and answers which are unsafe data. These are very less compared to the total training data. The model is then trained using SFT using this data. They show that using less data we can still have a malicious model which can jailbreak easily. \cite{Deng2023MASTERKEYAJ} trains a red model to generate automatic prompts based on the feedback of the target model.
% (persona assigned papers)
The work by \cite{Shah2023ScalableAT} investigates persona modulation as a black-box jailbreaking method to steer a target model to take on personalities that are willing to comply with harmful instructions.



\subsection{Stereotypical bias in LLMs}
\cite{Deshpande2023ToxicityIC} uses persona-based assignments to generate toxic contents from GPT models. Similar to this work, \cite{Gupta2023BiasRD} shows that that the practice of assigning personas to
LLMs—a trend on the rise—can surface their deep-rooted biases and have unforeseeable and detrimental side effects. 

\cite{Esiobu2023ROBBIERB} benchmarks different bias metrics and suggests mitigation strategies in context to the current state-of-the-art LLMs.  \cite{kotek2023gender} investigate how gender biases are reflected in the current LLMs and show how the LLMs rationalize for their biased behaviour. \cite{ma-etal-2023-intersectional} look at intersectional stereotypes which do not fit into a broad single-group category. 
